AALF: Almost Always Linear Forecasting

Recent works for time-series forecasting more and more leverage the high predictive power of Deep Learning models. With this increase in model complexity, however, comes a lack in understanding of the underlying model decision process, which is problematic for high-stakes application scenarios. At the same time, simple, interpretable forecasting methods such as ARIMA still perform very well, sometimes on-par, with Deep Learning approaches. We argue that simple models are good enough most of the time, and that forecasting performance could be improved by choosing a Deep Learning method only for few, important predictions, increasing the overall interpretability of the forecasting process. In this context, we propose a novel online model selection framework which learns to identify these predictions. An extensive empirical study on various real-world datasets shows that our selection methodology performs comparable to state-of-the-art online model selections methods in most cases while being significantly more interpretable. We find that almost always choosing a simple autoregressive linear model for forecasting results in competitive performance, suggesting that the need for opaque black-box models in time-series forecasting might be smaller than recent works would suggest.

==> plots/metrics_table_all.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} lrrrrrrrrrrrrrrr}
\toprule
 & Pedestrian & Web & KDD & Weather \\
\midrule
MeanValue & 1.024 & 1.872 & 0.568 & 0.954 \\
LastValue & 0.485 & 1.907 & 0.296 & 1.149 \\
AALF$_{0.5}$ & \textbf{0.287} & 1.433 & \underline{0.288} & \textbf{0.877} \\
AALF$_{0.6}$ & 0.291 & 1.436 & \textbf{0.288} & \underline{0.877} \\
AALF$_{0.7}$ & 0.299 & 1.433 & 0.288 & 0.879 \\
AALF$_{0.8}$ & 0.311 & 1.446 & 0.288 & 0.882 \\
AALF$_{0.9}$ & 0.335 & 1.455 & 0.289 & 0.889 \\
AALF$_{0.95}$ & 0.360 & 1.486 & 0.290 & 0.896 \\
AALF$_{0.99}$ & 0.397 & 1.627 & 0.292 & 0.903 \\
OMS-RoC & 0.289 & \underline{1.425} & 0.289 & 0.895 \\
KNN-RoC & 0.292 & 1.441 & 0.289 & 0.899 \\
ADE & 0.377 & 1.489 & 0.294 & 0.905 \\
DETS & \underline{0.287} & \textbf{1.395} & 0.288 & 0.891 \\
$f_i$ & 0.414 & 1.655 & 0.293 & 0.904 \\
$f_c$ & 0.289 & 1.433 & 0.290 & 0.901 \\
\bottomrule
\end{tabular*}

==> plots/table.tex <==
\begin{tabular}{lrr|rr|rr|rr|rr}
\toprule
 & \multicolumn{2}{c}{lin} & \multicolumn{2}{c}{nn} & \multicolumn{2}{c}{v12\_0.7} & \multicolumn{2}{c}{v12\_0.8} & \multicolumn{2}{c}{v12\_0.9} \\
 & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE \\
\midrule
Pedestrian & 0.258 & 0.168 & \textbf{0.181} & \textbf{0.098} & 0.203 & 0.104 & 0.216 & 0.110 & 0.232 & 0.121 \\
Web & 0.798 & 366.933 & 0.690 & 26.297 & \textbf{0.681} & \textbf{26.207} & 0.688 & 26.233 & 0.701 & 26.282 \\
KDD & 0.165 & \textbf{0.122} & 0.163 & 0.125 & \textbf{0.162} & 0.122 & 0.162 & 0.122 & 0.163 & 0.123 \\
Weather & 0.623 & 0.911 & 0.614 & 0.909 & \textbf{0.592} & \textbf{0.870} & 0.597 & 0.875 & 0.608 & 0.886 \\
\bottomrule
\end{tabular}

